ATLAS Upgrade Instrumentation in the US

Planned upgrades of the LHC over the next decade should allow the machine to operate at a center of mass energy of 14 TeV with instantaneous luminosities in the range 5--7e34 cm^-2 s^-1. With these parameters, ATLAS could collect 3,000 fb^-1 of data in approximately 10 years. However, the conditions under which this data would be acquired are much harsher than those currently encountered at the LHC. For example, the number of proton-proton interactions per bunch crossing will rise from the level of 20--30 per 50 ns crossing observed in 2012 to 140--200 every 25 ns. In order to deepen our understanding of the newly discovered Higgs boson and to extend our searches for physics beyond that new particle, the ATLAS detector, trigger, and readout will have to undergo significant upgrades. In this whitepaper we describe R&D necessary for ATLAS to continue to run effectively at the highest luminosities foreseen from the LHC. Emphasis is placed on those R&D efforts in which US institutions are playing a leading role.

==> Makefile <==
LATEX    = latex
BIBTEX   = bibtex
DVIPS    = dvips

BASENAME = atlas-instrum

default: testpdflatex

testlatex:
	latex  ${BASENAME}
	latex  ${BASENAME}
	bibtex ${BASENAME}
	latex  ${BASENAME}
	latex  ${BASENAME}
	dvipdf -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress ${BASENAME}

testpdflatex:
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}
	bibtex    ${BASENAME}
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}

#
# standard Latex targets
#

%.dvi:	%.tex 
	$(LATEX) $<

%.bbl:	%.tex *.bib
	$(LATEX) $*
	$(BIBTEX) $*

%.ps:	%.dvi
	$(DVIPS) $< -o $@

%.pdf:	%.tex
	$(PDFLATEX) $<

.PHONY: clean

clean:
	rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg  \
	      *.inx *.dvi *.toc *.out *~ ~* spellTmp 


